Select before Act: Spatially Decoupled Action Repetition for Continuous Control

Reinforcement Learning (RL) has achieved remarkable success in various continuous control tasks, such as robot manipulation and locomotion. Different to mainstream RL which makes decisions at individual steps, recent studies have incorporated action repetition into RL, achieving enhanced action persistence with improved sample efficiency and superior performance. However, existing methods treat all action dimensions as a whole during repetition, ignoring variations among them. This constraint leads to inflexibility in decisions, which reduces policy agility with inferior effectiveness. In this work, we propose a novel repetition framework called SDAR, which implements Spatially Decoupled Action Repetition through performing closed-loop act-or-repeat selection for each action dimension individually. SDAR achieves more flexible repetition strategies, leading to an improved balance between action persistence and diversity. Compared to existing repetition frameworks, SDAR is more sample efficient with higher policy performance and reduced action fluctuation. Experiments are conducted on various continuous control scenarios, demonstrating the effectiveness of spatially decoupled repetition design proposed in this work.

==> tmp.tex <==
\begin{table}[t]
\caption{
Episode return of each method in different task environments.
The best results are boldfaced.
Our method SDAR outperforms baseline methods generally, with minor performance reductions observed in \emph{LunarLander} and \emph{Pusher}.
More results in other tasks are given in Appendix~\ref{app:exp_res_results_of_return}.
}
\begin{center}
\begin{small}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Task} & \multicolumn{6}{c}{Episode Return}  \\
\cmidrule{2-7}
& SAC & N-Rep & TempoRL & TAAC & UTE & SDAR (Ours) \\ 
\midrule
LunarLander & 275.9$\pm$6.83 & 280.8$\pm$1.21 & 281.5$\pm$7.22 & 261.4$\pm$18.9 & \textbf{282.8$\pm$8.74} & 282.2$\pm$5.84 \\ 
Walker2d & 5305$\pm$367 & 4724$\pm$163 & 2866$\pm$897 & 5660$\pm$394 & 2986$\pm$836 & \textbf{6028$\pm$406} \\ 
HalfCheetah & 13122$\pm$2877 & 8378$\pm$1753 & 8065$\pm$1799 & 11148$\pm$3921 & 7917$\pm$293 & \textbf{15131$\pm$1279} \\ 
Humanoid & 6184$\pm$717 & 5074$\pm$310 & 1022$\pm$397 & 7308$\pm$244 & 2595$\pm$334 & \textbf{7483$\pm$288} \\ 
Pusher & -22.5$\pm$1.40 & \textbf{-21.2$\pm$1.08} & -48.2$\pm$2.05 & -30.5$\pm$1.85 & -41.3$\pm$5.56 & -21.3$\pm$1.26 \\ 
\midrule
\textbf{Normalized} & 0.89$\pm$0.07 & 0.81$\pm$0.19 & 0.59$\pm$0.33 & 0.91$\pm$0.10 & 0.64$\pm$0.27 & \textbf{1.00$\pm$0.001} \\ 
\bottomrule
\end{tabular}
\end{small}
\end{center}
\label{tab:exp_results_return}
\end{table}

\begin{table}[t]
\begin{center}
\caption{
Experiment results of APR and AFR in different tasks, where AFR results are given in square brackets.
As illustrated in Table~\ref{tab:exp_results_return} and Table~\ref{tab:exp_results_fluctuation}, \alg{SDAR} achieves excellent performance on action persistence and action fluctuation, while outperforms other methods on episode return.
}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Task} & \multicolumn{6}{c}{Action Persistence Rate \& [Action Fluctuation Rate]}  \\
\cmidrule{2-7}
& SAC & N-Rep & TempoRL & TAAC & UTE & SDAR \\ 
\midrule
LunarLander & 1.0[0.09] & 4.0[0.08] & 1.43[0.18] & 3.05[0.11] & 1.38[0.36] & 11.18[0.10] \\ 
Walker2d & 1.0[0.15] & 4.0[0.09] & 5.74[0.26] & 1.30[0.22] & 7.81[0.24] & 2.96[0.12] \\ 
HalfCheetah & 1.0[0.68] & 2.0[0.47]  & 2.10[0.66]  & 1.02[0.61]  & 2.69[0.58]  & 1.22[0.62]  \\ 
Humanoid & 1.0[0.28] & 4.0[0.09] & 5.27[0.15] & 1.21[0.25] & 5.69[0.18] & 1.67[0.19] \\ 
Pusher & 1.0[0.022] & 4.0[0.008]  & 1.15[0.032]  & 1.75[0.031]  & 1.01[0.018]  & 1.69[0.015]  \\ 
\midrule
\textbf{Average} & 1.0[0.245] & 3.6[0.148]  & 3.12[0.257]  & 1.66[0.244]  & 3.71[0.276]  & 3.75[0.208]  \\ 
\bottomrule
\end{tabular}
\end{center}
\label{tab:exp_results_fluctuation}
\end{table}

